MultiGraphMatch: a subgraph matching algorithm for multigraphs

Subgraph matching is the problem of finding all the occurrences of a small graph, called the query, in a larger graph, called the target. Although the problem has been widely studied in simple graphs, few solutions have been proposed for multigraphs, in which two nodes can be connected by multiple edges, each denoting a possibly different type of relationship. In our new algorithm MultiGraphMatch, nodes and edges can be associated with labels and multiple properties. MultiGraphMatch introduces a novel data structure called bit matrix to efficiently index both the query and the target and filter the set of target edges that are matchable with each query edge. In addition, the algorithm proposes a new technique for ordering the processing of query edges based on the cardinalities of the sets of matchable edges. Using the CYPHER query definition language, MultiGraphMatch can perform queries with logical conditions on node and edge labels. We compare MultiGraphMatch with SuMGra and graph database systems Memgraph and Neo4J, showing comparable or better performance in all queries on a wide variety of synthetic and real-world graphs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> reviewer.tex <==
\section*{Reviewer Comments and Responses}

First we would like to thank the reviewers for their insightful comments. We have improved the paper thanks to those comments. All our modifications to the text are highlighted in red within the paper. Below, we copy each comment and then describe how we have responded to it.

\subsection*{Reviewer 1}

\subsubsection*{Major comments}

\begin{enumerate}

\item (Part 1) The major concern I have with this paper is that it introduces a wide variety of techniques for processing multigraph matchings (the bit signature, the ordering, the symmetry breaking), but I have no sense for why this algorithm performs better than other algorithms which exist in the literature. The other algorithms I'm sure also make some consideration in terms of candidate elimination and ordering as well, so it would be nice to hear some insight from the authors as to why their proposed method works better. I can see from the experimental results that it does, but some examples or other kinds of tests may help elucidate where the improvement is coming from. As this paper is already fairly wrong, I don't expect a new set of experiments, but I hope at least some thought is given to this.\\ (Part 2) The major concern that I have with this paper is that I struggle to find what is the novel contribution that demonstrates that this given algorithm improves upon the other subgraph matching algorithms that exist in the literature. The authors present some new data structure, the “bit signature” and a way of ordering, but I would like to see some insight if possible which explains why these particular methods are so good beyond numerical experiments (which are good too!). The subgraph matching literature is full of a variety of different methods and data structures for eliminating candidate vertices in a match and determining the ordering of processing of vertices and edges. This paper would be improved if it could expound upon why the current methods for multigraph matching are lacking and how this new algorithm addresses those concerns. In fact, if the authors could illustrate some example instances (either synthetic or from actual problems) which show how the proposed methods improve, it would help distinguish this method from the rest.\\\\
\color{blue}
We thank the reviewer for these three important points. 
First, concerning the use of classical subgraph matching algorithms, we explain in the Introduction (Section \ref{introduction}) that these algorithms, which are designed for simple graphs, only support the equality operator on labels. Through an example on a clique, we demonstrate that applying any of these algorithms to multigraphs results in a post-processing step on top of an exponential number of candidate occurrences that have to be filtered, while MultiGraphMatch is quadratic in query nodes and target nodes.

Second, we extended the ablation studies presented in Section \ref{ablationExp} to show that the novel scoring function we designed that combines minimization of domain cardinalities and maximization of node degrees based on Jaccard similarity can lead to a significant improvement of performance (especially for tree-like topologies) with respect to a scoring function based solely on minimization of domain cardinalities, which has been commonly used as a scoring function in many state-of-the-art subgraph matching algorithms. 

Third, ablation tests (Section \ref{ablationExp}) and scalability tests on LDBC benchmark (Section \ref{scalabilitySec}) demonstrate that the novel bit matrix is an effective (also fast) data-structure to prune the set of candidates for matching, representing a good compromise between filtering power and memory consumption.
\color{black}


\end{enumerate}

\subsubsection*{Minor comments}

\begin{enumerate}

\item Page 2, Lines 31-39: There is a distinction made between “labeled” graphs and “attributed” graphs in the introduction. What is the difference between labels and attributes? Why is the community a person belongs to a label and their age an attribute? Further down the page, you use the term “property.” Is this a label or is this an attribute or something else? \\\\
\textcolor{blue}{Yes, this was unnecessarily complicated. In the Introduction (Section \ref{introduction}), in the definition of attributed graph, we replaced the term “attribute” with “property” as the term “attribute” was defined only once in the Introduction. Next, we clarified the difference between “label” and “property”.}\\

\item Page 2, Line 46: Make sure to use right-facing quotes, ’actor’ vs. ‘actor’ \\\\
\textcolor{blue}{We fixed the notation in the Introduction (Section \ref{introduction}), also for the terms “director”, “directed” and “acted\_with”.}\\

\item Page 5, Line 27: What is L+? \\\\
\textcolor{blue}{In the Preliminary Definitions section (Section \ref{definitions}), we replaced L+ with $P(L) \setminus \{ \emptyset \}$, where P(L) is the power-set of L. At the beginning of the Preliminary Definitions section, we also explicitly explained what P(.) stands for.}\\

\item Page 5, Line 29: What is an edge type? What is the difference between a type, a label, an attribute, and a property? Is there any difference? \\\\
\textcolor{blue}{In the Preliminary Definitions section (Section \ref{definitions}) we modified the text by stating that T is the set of edge labels, which are also called types. The term “attribute” is used only once, in the Introduction, and, as reported in the previous minor comment 1, is synonymous with “property”. In addition to the Introduction section, the distinction between “label” and “property” was re-stated also in the Preliminary Definitions section.}\\

\item Page 5, Lines 31-34: Issues with notation, A : N → PN ×VN. I believe N written here should be V , the set of nodes. Also, you write that each node will be associated with a set of property-value pairs, in which case the codomain of A should be P(PN ×VN), the power set of PN ×VN. As it is, the output of A is just a single pair. Similar issues hold for B \\\\
\textcolor{blue}{In the Preliminary Definitions section (Section \ref{definitions}), we replaced set N with set V. We also replaced the set of values V\_N and V\_E with X\_V and Y\_E, respectively, to avoid confusion with the set of graph nodes V and changed the codomain of the property assignment functions to the power set P of the property-values pairs.}\\

\item Page 5: Further notation issues regarding the edge set E. If E is simply a set of ordered pairs (u, v), then there is no possibility for multiple edges. Furthermore, you say a graph is undirected if $(u, v) \in E$ implies $(v, u) \in E$. However, in a world where there are multiple edges and edges have labels (types?), you wouldn’t say a graph is undirected if there are three edges going one way and two the other way.\\\\
\textcolor{blue}{We thank the reviewer for this important observation. We addressed this point in the Preliminary Definitions section (Section \ref{definitions}). We defined an edge as a triplet formed by a unique identifier, the source and the destination node. We also removed the definition of “undirected” graphs.}\\

\item Page 6: An extension of the previous point, if we have multiple edges in the query, we should want them to be mapped to different edges in the target. (1) of the definition of submultigraph matching doesn’t appear to make the distinction between different edges between the same vertices.\\\\
\textcolor{blue}{We agree with this observation. In the Preliminary Definitions section (Section \ref{definitions}), we modified  condition (1) of the definition of submultigraph matching, so that now the same query edge can be matched with different edges between two target nodes.}\\

\item Page 6, Lines 32-33: I assume (p : v) should be (p, v), otherwise I am not sure what (p : v) means.\\\\
\textcolor{blue}{We fixed the notation in the Preliminary Definitions section (Section \ref{definitions}).}\\

\item Page 6, lines 40-41: “Given an edge mapping g, an occurrence of Q in T is a graph O formed by edges g(e1), g(e2), . . . , g(ek) where all nodes that are sources or destinations of at least one of these edges.” This is an incomplete sentence. I am not sure what this means.\\\\
\textcolor{blue}{We have addressed this point by replacing the word “where” with the word “and” in the Preliminary Definitions section (Section \ref{definitions}).}\\

\item Page 7, Lines 10-11: It mentions supplementary material with Cypher syntactic constructs. Where can I find this?\\\\
\textcolor{blue}{We thank the reviewer for this important point. We included the list of constructs supported by MultiGraphMatch in a PDF file and upload the PDF file in our GitHub repo (https://github.com/Anto188bas/MultiGraphMatch.git). Therefore  users who want to use our software can learn the  syntax of CYPHER queries that should be provided as input to MultiGraphMatch. We also added a reference to the GitHub repo in the Cypher Query Language section (Section \ref{cypher}).}\\

\item Page 7, Line 28-29: “Edges are specified by line or curve segments that may or may not have an arrowhead”. I assume this is referring to the characters which are used to specify an edge in the CYPHER language, but I am not sure what a line or curve segment would be?\\\\
\textcolor{blue}{We clarified this point in the Cypher Query Language section (Section \ref{cypher}), by specifying that edges can be connected to nodes using either the string “-” or the strings “<-” and “->” depending on whether a particular edge is bidirectional or directional.}\\

\item Page 8, Lines 45-49: Can you be clearer about what the node labels graph is? Do we have a vertex for each possible subset of labels which appear in a graph? Also, you say it is a labeled graph, what are the labels?\\\\
\textcolor{blue}{This is a good point. To address this, we detailed and clarified the structure of the node labels graph in the "Indexing of target network" section (Section \ref{IndexingSec}).}\\

\item Page 11: Some additional references on symmetry breaking for subgraph matching: There are two algorithms, ISMA and ISMAGS (which is an extension of ISMA for general automorphisms). References listed below:
Demeyer, S., Michoel, T., Fostier, J., Audenaert, P., Pickavet, M., and Demeester, P. (2013). The index-based subgraph matching algorithm (ISMA): fast subgraph enumeration in large networks using optimized search trees. PloS one, 8(4), e61183.
Houbraken, M., Demeyer, S., Michoel, T., Audenaert, P., Colle, D., and Pickavet, M. (2014). The Index-based Subgraph Matching Algorithm with General Symmetries (ISMAGS): exploiting symmetry for faster subgraph enumeration. PloS one, 9(5), e97896.
Another recent paper on symmetry in subgraph matching: 
Yang, D., Ge, Y., Nguyen, T., Molitor, D., Moorman, J. D., and Bertozzi, A. L. (2023). Structural equivalence in subgraph matching. IEEE Transactions on Network Science and Engineering.\\\\
\textcolor{blue}{ We have added citations to these useful papers in the "Computation of symmetry breaking conditions" section (Section \ref{breakingCondSec}).}\\

\item Page 12, line 45: ”where $\land$ is the bitwise operator“ should be ”where $\land$ is the bitwise and operator“\\\\
\textcolor{blue}{We fixed the typo in the "Computation of compatibility domains" section (Section \ref{CompDomainsSec}).}\\

\item Page 11-13: In computing the compatibility domains, you only check for a given edge type if there exists an edge of a certain type between vertices. Is there a reason you don’t also check for if there are enough edges of a given type to support the number of edges between vertices in the query? This seems like it wouldn’t be difficult to add and would be useful in checking compatibility.\\\\
\textcolor{blue}{Thanks for pointing this out. We clarified this concept in the "Computation of compatibility domains" section (Section \ref{CompDomainsSec}), by explaining that type multiplicities in multiple edges connecting two nodes are actually taken into account to build compatibility domains when filtering using type-dependent degrees. This filtering phase follows the filtering of candidates based on bit matrices that just record the presence or absence of a specific edge type between two nodes.}\\

\item Page 17, Line 25: What is lT ? Is it supposed to be defined to be |LT |? If so, it should be phrased differently, using “If |LT | = lT ” appears to be setting up a conditional statement.\\\\
\textcolor{blue}{We rephrased the sentence as “Let |LT | = lT” in the "Complexity analysis" section (Section \ref{complexitySec}) and separated it from the following statement, to clarify that this is a general assumption and not a conditional statement.}\\

\item Page 17, Lines 33-36: When you discuss the complexity of computing automorphisms, you need to be a little more precise than you are. Computing graph isomorphism itself is not known to be P or NP-complete, and without knowing that $P \neq NP$, we cannot assert that we require O(2nQ) to solve the graph isomorphism problem. Also, I think you are using O(2nQ) as a shorthand for exponential time algorithms which is not quite right since exponential algorithms with different bases are in different complexity classes $(O(2n) \neq O(3n))$. If you want to include the complexity for computing the automorphism group, it would be better to have a precise accounting of what the complexity is as well as a citation for where this complexity comes from.\\\\
\textcolor{blue}{We  thank the reviewer for the comment. We addressed this in the "Complexity analysis" section (Section \ref{complexitySec}), by clarifying that graph isomorphism is not known to be NP-complete or not, but the algorithm we use to compute automorphism, NAUTY, requires $O(\exp(n\_Q))$ in the worst case, as proven in a previous work by Miyazaki in 1997 that we cite in our paper.}\\

\item Page 19-: It is not entirely clear to me what experiment that you are running. Are you trying to produce all subgraphs which match a given query or just a single one?\\\\
\textcolor{blue}{At the beginning of the "Experimental Results" section (Section \ref{experiments}), we specified that all performed experiments consist in counting all the occurrences of a given query graph in a target.}\\

\item Page 19, line 37: How did you extract query graphs from the networks? Randomly selected nodes? Random walks? Something else?\\\\
\textcolor{blue}{We thank the reviewer for the point. We illustrated the random-walk based algorithm we use to extract queries in the subsection about the performance comparison of synthetic networks (Section \ref{performanceSynthetic}). We also specified that the same algorithm was used for the experiments on real networks too (Section \ref{performanceReal}).}\\

\item Page 19, Line 38: What does density mean for multigraphs?\\\\
\textcolor{blue}{We defined the concept of density in the subsection of performance comparison of synthetic networks (Section \ref{performanceSynthetic}), where the concept is introduced for the first time.}\\

\item Page 20-21, Figures: Figures should include units! I assume that they are all in seconds but it needs to be stated.\\\\
\textcolor{blue}{We specified the time unit in all figures and tables and their captions both in the main paper and in the appendix.}\\

\item Page 21, Line 46: What are fractal networks?\\\\
\textcolor{blue}{We fixed the typo in Section \ref{performanceSynthetic}, by replacing “fractal” with “power-law”. In addition, at the beginning of Section \ref{syntheticdatasets} we specified that labels were generated with a power-law distribution having exponent $-1.2$.}\\

\end{enumerate}


\subsection*{Reviewer 2}

\begin{enumerate}

\item In the introduction, the "citation [21,21,31,37]" is duplicated in Line 104.\\\\
\textcolor{blue}{We fixed the typo in the "Introduction" section (Section \ref{introduction}).}\\

\item It would be valuable to elaborate on why conventional subgraph matching algorithms [36] cannot be directly adapted to the SMM problem and to highlight the challenges that arise in attempting to do so. Alternatively, addressing the performance limitations of these algorithms when applied to the SMM scenario would enhance the paper.
[36]: In-Memory Subgraph Matching: An In-Depth Study. \\\\
\textcolor{blue}{We  thank the reviewer for the interesting comment. We addressed this in the "Introduction" section (Section \ref{introduction}) by explaining that classical subgraph matching algorithms that work on simple graphs support only single labels on edges. By using any of these algorithms, the matching time requires exponential time. We have also added a figure with an example that depicts such a case.}\\

\item Consider utilizing a more recent baseline in place of SumGra.\\\\
\textcolor{blue}{We thank the reviewer for the comment. We added in the "Introduction" section (Section \ref{introduction}) a reference to a recent paper by Anwar et al. (Mathematics, 2022) and in the "Related Works" section (Section \ref{related}) a brief description of their algorithm. They compare their algorithm with SuMGra, but the set of proposed experiments is limited to very small networks (1,000 times smaller than the networks tested in our experiments) and the improvement over SuMGra is small. In addition, authors did not provide any source code or executable of their algorithm.}\\

\item The new scoring method introduced in the article claims to provide a more precise estimation of cardinality. To substantiate this assertion, it is essential to include theoretical explanations or experimental data supporting this claim. Merely analyzing time metrics may not sufficiently validate the effectiveness of the new scoring approach.\\\\
\textcolor{blue}{Thank you for this useful comment. To address this, we extended the ablation tests (Section \ref{ablationExp}) to include a set of experiments where MultiGraphMatch is run with a scoring function based solely on minimization of domain cardinalities. The experiments show that in general using our scoring function that combines domain cardinalities with Jaccard similarities is  slightly better, but for specific types of queries (tree-like topologies) there is a significant improvement. In addition, at the end of Section \ref{ordering}, we show that in some cases domain cardinalities alone are not enough to derive a good ordering, because starting from a query edge involving high-degree nodes (even though the cardinality of its domain is not the minimum one) can produce a better ordering leading to an earlier and indeed more effective pruning of the search space during matching.}\\

\end{enumerate}


==> reviewer_v2.tex <==
\section*{Reviewer Comments and Responses}

We would like to thank the reviewers for their useful comments that further improved the paper. All our modifications to the text are highlighted in red within the paper. Below, we copied each comment and described how we responded to them.

\subsection*{Reviewer 1}

\begin{enumerate}

\item In Section 6.1.3, Page 22, the random ordering is not a good option for comparison. Using an existing ordering would be more convincing in demonstrating the advantages of the minimization of domain cardinalities.\\

\color{blue}

We thank the reviewer for this important point. To the best of our knowledge, in the context of sub-multigraph matching, there is no existing scoring function for edges that is ready to be used. Concerning subgraph matching in simple graphs, proposed scoring functions mainly take into account the following criteria: node degrees, frequency of edge labels in the target and cardinalities of candidate sets. For this reason, we decided to integrate our ablation tests (Section \ref{ablationExp}) with two additional versions of MultiGraphMatch: MGM-EL, in which the scoring function is based solely on the frequency of query edge labels in the target, and MGM-DE, in which the scoring function takes into account only the numerator of the $Sc$ score defined in Section \ref{ordering}, which is related to the degrees of the edge's endpoints. Please note that cardinalities of candidate sets have already been taken into account in the MGM-MDC version of MultiGraphMatch, in which the ordering is computed based on minimization of compatibility domains.\\

\color{black}

\item In Section 1, it said that the results of subgraph matching should be post-processing in exponential time. I believe that existing subgraph matching algorithms can also filter node pairs in $O(k^2n^2)$ to eliminate the need for post-processing. For example, in DAF [20] matching, during CS Structure, the edge labels could be considered, although the algorithms do not specify how to find matches when edges have labels.
The limitations of using SM in SMM should be further discussed. For example, What is the overhead or the difficulty in modifying existing subgraph matching algorithms to accommodate edge labels?\\

\color{blue}

We thank the reviewer for this useful comment. We revised the complexity analysis regarding matching and post-processing of existing subgraph matching algorithms that work only on simple graphs (Section \ref{introduction}, page 3). We show that, in general, such algorithms need post-processing, even in presence of filtering data structures that handle edge labels, but these post-processing operations do not require exponential time. By contrast, algorithms specifically designed to work on multigraphs, such as MultiGraphMatch, can find the correct mapping between query and target edges during matching, so they do not need to post-process the results.\\

\color{black}

\item The main contributions listed in Section 1 could be better for readers.\\

\color{blue}

We thank the reviewer for the point. To help the reader, the main contributions of the paper have been now synthesized in the form of an item list in Section \ref{introduction} page 4, emphasizing the novel algorithmic ideas introduced by MultiGraphMatch. \\

\end{enumerate}

\color{black}


\subsection*{Reviewer 2}

\begin{enumerate}

\item Only one small issue that I have with the changes. On page 6, the edges are taken from $N \times V \times V$, where I assume N is now a set of identifiers for edge, but N is never defined. Also further down the page in the definition for multigraph matching, I think it should be explicitly stated that for e = (x, u,v), that the output of the edge mapping g(e) is an edge of the target. This is implicitly true by the fact that the codomain of g is the set of edges of the target, but I think it is helpful to make clear that adjacent vertices in the query are mapped to adjacent vertices in the target.\\

\color{blue}

We thank the reviewer for the comment. In the two definitions reported in Section \ref{definitions} pages 6 and 7, we specified that N is the set of unique edge identifiers and g(e) belongs to the set of target edges. In the definition of submultigraph matching on page 7, we also clarified why condition 1 ensures that edge mapping is consistent with node mapping.\\

\color{black}

\end{enumerate}

==> temp.tex <==
Algorithms \ref{CheckNodeCond_Algo} and \ref{CheckEdgeCond_Algo} detail how MultiGraphMatch checks whether breaking conditions on nodes and edges are satisfied, respectively. Given the partial node mapping function $f$ and a candidate target node $t$ to be mapped with a query node $q$, MultiGraphMatch considers the set of all breaking conditions (if any) involving $q$ (Algorithm \ref{CheckNodeCond_Algo}). For each such breaking condition $q' \prec q$, the algorithm checks whether $id(f(q))<id(t)$. If, for at least one of these conditions, $id(f(q))>id(t)$ (i.e. the breaking condition is violated), the algorithm stops and returns a negative response. A similar procedure is followed in Algorithm \ref{CheckEdgeCond_Algo} to check symmetry breaking conditions on a target edge, given the set of target edges that have been already mapped through the edge mapping function $g$. 

%\IncMargin{1em}
%\begin{algorithm}
%\label{CheckNodeCond_Algo}
%\KwIn{$\mathcal{BC}_N$: set of symmetry breaking conditions on nodes, $q$: query node, $t$: target node, $f$: current node mapping}
%\KwOut{$Res$: boolean response}
%\SetKw{Kw}{break}
%$Res := true$\;
%\ForEach{$q' \prec q \in \mathcal{BC}_N(q)$}{
%    \uIf{$f(q') != undefined \land id(f(q'))>id(t)$}{
%        $Res := false$\;
%        \Kw{}
%    }
%}
%\KwRet{$Res$}
%\caption{\textsc{CheckNodeBreakingCond}($\mathcal{BC}_N,q,t,f$)}
%\end{algorithm}

%\IncMargin{1em}
%\begin{algorithm}
%\label{CheckEdgeCond_Algo}
%\KwIn{$\mathcal{BC}_E$: set of symmetry breaking conditions on edges, $e_Q$: query edge, $e_T$: target edge, $g$: current edge mapping}
%\KwOut{$Res$: boolean response}
%\SetKw{Kw}{break}
%$Res := true$\;
%\ForEach{$e'_Q \prec e_Q \in \mathcal{BC}_E(e_Q)$}{
%    \uIf{$g(e'_Q) != undefined \land id(g(e'_Q))>id(e_T)$}{
%        $Res := false$\;
%        \Kw{}
%    }
%}
%\KwRet{$Res$}
%\caption{\textsc{CheckEdgeBreakingCond}($\mathcal{BC}_E,e_Q,e_T,g$)}
%\end{algorithm}
